Probabilistic Programming with Programmable Variational Inference

Compared to the wide array of advanced Monte Carlo methods supported by modern probabilistic programming languages (PPLs), PPL support for variational inference (VI) is less developed: users are typically limited to a predefined selection of variational objectives and gradient estimators, which are implemented monolithically (and without formal correctness arguments) in PPL backends. In this paper, we propose a more modular approach to supporting variational inference in PPLs, based on compositional program transformation. In our approach, variational objectives are expressed as programs, that may employ first-class constructs for computing densities of and expected values under user-defined models and variational families. We then transform these programs systematically into unbiased gradient estimators for optimizing the objectives they define. Our design enables modular reasoning about many interacting concerns, including automatic differentiation, density accumulation, tracing, and the application of unbiased gradient estimation strategies. Additionally, relative to existing support for VI in PPLs, our design increases expressiveness along three axes: (1) it supports an open-ended set of user-defined variational objectives, rather than a fixed menu of options; (2) it supports a combinatorial space of gradient estimation strategies, many not automated by today's PPLs; and (3) it supports a broader class of models and variational families, because it supports constructs for approximate marginalization and normalization (previously introduced only for Monte Carlo inference). We implement our approach in an extension to the Gen probabilistic programming system (genjax.vi, implemented in JAX), and evaluate on several deep generative modeling tasks, showing minimal performance overhead vs. hand-coded implementations and performance competitive with well-established open-source PPLs.

==> 01introduction_backup.tex <==
\section{Introduction}
\label{sec:intro}

\textit{Variational inference} (VI) problems are optimization problems in spaces of probability distributions. Variational inference algorithms have found widespread adoption both in Bayesian settings, where the goal is to find an accurate approximation to an intractable posterior~\citep{fox2012tutorial,kucukelbir2017automatic,blei2017variational,hoffman2013stochastic,blei2006variational}, and in deep learning, where the goal is to fit neural, latent-variable generative models% to data
~\cite{kingma_auto-encoding_2022,pu2016variational,kingma2021variational,vahdat2020nvae,malkin2022gflownets}. %To face problems of growing complexity, researchers have developed increasingly sophisticated approximations~\cite{agakov_auxiliary_2004,gu_neural_2015,kingma2013auto,maaloe_auxiliary_2016,eslami_attend_2016,le_inference_2017,malkin2022gflownets}, and objective functions~\cite{dempster_maximum_1977,hinton_wake-sleep_1995,agakov_auxiliary_2004,bornschein_reweighted_2015,burda_importance_2016,ranganath_hierarchical_2016,rainforth_tighter_2018,sobolev_importance_2019,malkin2022gflownets} to train approximations.

Unfortunately, implementing variational inference by hand can be tedious and error-prone. %Consider, for example, optimizing the ELBO ($Q \mapsto \mathbb{E}_{x \sim Q}[\log \frac{\tilde{p}(x)}{q(x)}]$), a common variational objective, by gradient descent. 
The typical variational inference problem is defined by three mathematical ingredients: a family of \textit{model distributions} $\mathcal{P} = \{P_\theta \mid \theta \in \RR^n\}$, a family of inference distributions $\mathcal{Q} = \{Q_\phi \mid \phi \in \RR^m\}$ (the \textit{variational family}), and a scalar \textit{objective function} $\mathcal{F} : \mathcal{P} \times \mathcal{Q} \to \mathbb{R}$ mapping particular distributions $P_\theta$ and $Q_\phi$ to a scalar \textit{loss} (or \textit{reward}). 
The goal of variational inference algorithms is to find parameters $\theta$ and $\phi$ which optimize $\mathcal{F}(P_\theta, Q_\phi)$. %The objective function is used to measure some kind of distance between the $P$ and $Q$ distributions,\footnote{Different notions of distance induce approximation solutions with different behavior: for instance, when using a variational algorithm to approximate an intractable posterior with a variational family that doesn't contain the true posterior, ELBO-based solutions are known to \textit{underestimate} the support of the posterior ("mode seeking" solutions), by virtue of the fact that ELBO optimization is equivalent to minimizing $KL(Q, \tilde{P})$, which is infinite when $\textbf{density}\{Q\}(z) > 0$ and $\textbf{density}\{\tilde{P}\}(z) = 0$. Optimization targeting the forward $KL(\tilde{P}, Q)$ induces the opposite behavior.} like the distance between $Q_\phi$ and a normalized posterior $\tilde{P}_\theta$ induced by conditioning $P_\theta$ on data, or the distance between the marginal of $P_\theta$ and an empirical data distribution. Common target objective functions\footnote{Each of which has seen modification or approximation to produce new variational algorithms~\cite{agakov_auxiliary_2004,bornschein_reweighted_2015,ranganath_hierarchical_2016,li_renyi_2016,kingma_auto-encoding_2022,le_revisiting_2019,zimmermann_nested_2021,gu_neural_2015,kim_markov_2022}.} include the evidence lower bound (ELBO)~\cite{jordan_introduction_1999,blei2017variational}, the forward Kullback–Leibler divergence (KL)~\cite{hinton_wake-sleep_1995,naesseth_markovian_2020}, and the log marginal likelihood (LML)~\cite{dempster_maximum_1977,hinton_wake-sleep_1995}: their definitions typically involve integration, density computations, and other operations on the distributions $P_\theta$ and $Q_\phi$.
%{\small\begin{align*}
%\mathcal{F}_\text{ELBO}(P_\theta, Q_\phi) := \mathbb{E}_{z \sim Q_\phi}[\log \frac{\textbf{density}\{P_\theta\}(x, z)}{\textbf{density}\{Q_\phi\}(z)}]&, \quad \mathcal{F}_{\text{fwd-KL}}(\tilde{P}_\theta, Q_\phi) := \mathbb{E}_{z \sim \tilde{P}_\theta}[\log \frac{\textbf{density}\{\tilde{P}_\theta\}(z)}{\textbf{density}\{Q_\phi\}(z)}] \\[5pt] \vspace{0.3in} \mathcal{F}_\text{LML}(P_\theta) := \log \textbf{density}\{&\textbf{marginal}_x\{ P_\theta \}\}(x)
%\end{align*}}
But when implementing variational inference algorithms by hand, neither $\mathcal{P}$, $\mathcal{Q}$, nor $\mathcal{F}$ are represented directly in code; rather, one must: 
%Optimizing these objective functions with respect to the continuous parameters of $P$ and $Q$ motivates the usage of gradient automation, but none of these ingredients are necessarily represented directly in code, and conventional automatic differentiation (AD) tools fail to account for their semantics~\cite{lew_adev_2023}.

% \vspace{0.05in}
% \noindent To implement a new algorithm, the practitioner must instead:
% Consider, for example, the common practice of optimizing a variational objective by stochastic gradient descent. The typical practitioner's workflow might comprise four steps:
\begin{enumerate}[leftmargin=*]
% \item Define a \textit{variational family}: a parametric class $\{Q_\theta \mid \theta \in \mathbb{R}^n\}$ of distributions to search over.
% \item Define a real-valued objective function $Q \mapsto \mathcal{L}(Q)$ to optimize. For example, $\mathcal{L}$ might be the KL divergence of $Q$ to another distribution $P$ ($\mathcal{L}(Q) = \mathbb{E}_{x \sim Q}[\log \frac{p(x)}{q(x)}]$).
\item use algebra, probability theory, and calculus to derive a \textit{gradient estimator}: a way to rewrite the gradient $\nabla_{(\theta, \phi)} \mathcal{F}(P_\theta, Q_\phi)$ as an expectation $\mathbb{E}_{y \sim M_{(\theta,\phi)}}[f_{(\theta, \phi)}(y)]$, for some family of distributions $M$ and some family of functions $f$; and then
\item write code to sample $y \sim M_{(\theta,\phi)}$ and evaluate $f_{(\theta, \phi)}(y)$\textemdash an unbiased estimate of $\nabla_{(\theta,\phi)} \mathcal{F}(P_\theta, Q_\phi)$.
%\item Run stochastic gradient descent, using unbiased gradient estimates obtained by sampling $x \sim M_\theta$ and evaluating $f_\theta(x)$. 
\end{enumerate}
It is often non-trivial to ensure that $M$ and $f$ are faithfully implemented, and that the math used to derive them in the first place is error-free. Small changes to $\mathcal{F}$, $\mathcal{P}$, or $\mathcal{Q}$, or to the gradient estimation strategy employed in step (1), can require large, non-local changes to $M$ and $f$, and in implementing these changes, it is easy to introduce hard-to-detect bugs. When optimization fails, it is often unclear whether the problem is with the math, the code, or just the hyperparameters.
%\vspace{-2mm}

\paragraph{Existing automation.} Reflecting the importance of variational inference, many probabilistic programming languages (PPLs) (especially ``deep'' PPLs, such as Pyro~\cite{bingham_pyro_2018}, Edward~\cite{tran_2017_deep,tran2018simple}, and ProbTorch \cite{stites_learning_2021}), feature varying degrees of automation for VI workflows. In these languages, users can express both models $\mathcal{P}$ and variational families $\mathcal{Q}$  as probabilistic programs; the system then automates the estimation of gradients for a pre-defined set of supported variational objectives $\mathcal{F}$. This design significantly lowers the cost of implementing and iterating on variational inference algorithms, but several pain points remain:  %selected from a pre-defined menu of options. %Early implementations relied on black-box variational inference~\cite{ranganath_black_2014}, But recent years have seen many improvements: for example, Pyro~\cite{bingham_pyro_2018} supports an impressive roster of roster of variational objectives and gradient estimation strategies. But they do so via a {menu-based} approach: users can freely specify $\mathcal{P}$ and $\mathcal{Q}$ as probabilistic programs, but then must choose from a pre-defined set of options for the variational objective $\mathcal{F}$. Each objective in turn supports only limited customization of the strategy for estimating its gradient. This approach has several drawbacks:
\begin{itemize}[leftmargin=*]
\item \textbf{Incomplete coverage.} Many variational objectives and gradient estimation strategies are not supported by today's PPLs. For example, existing PPLs offer limited or no support for forward KL objectives~\cite{naesseth_markovian_2020}; hierarchical, nested, or recursive variational objectives~\cite{ranganath_hierarchical_2016,zimmermann_nested_2021,lew_recursive_2022}; symmetric divergences~\cite{domke_easy_2021}; trajectory-balance objectives~\cite{malkin2022gflownets}; SMC-based objectives~\cite{maddison_filtering_2017,gu_neural_2015,li_neural_2023,naesseth2018variational}; and others. Today's PPLs also do not automate many powerful gradient estimation strategies, for example those based on measure-valued differentiation~\citep{mohamed2020monte}.
%\item \textbf{Incomplete coverage (gradient estimators).} Even when the user's desired variational objective is supported, it may not implement the gradient estimation strategy that the user wants to apply. For example, Pyro supports importance-weighted objectives~\cite{burda_importance_2016} (\texttt{RenyiELBO}), but uses high-variance gradient estimators~\cite{williams_simple_1992} to handle discrete variables in the variational family. Variance reduction strategies like data-dependent baselines or enumeration, although implemented as parts of other menu options, cannot be applied with importance-weighted objectives.
\item \textbf{Duplicative engineering effort.} For PPL maintainers, supporting new gradient estimation strategies or language features requires separately introducing the same logic into the implementations of multiple variational objectives. Because this engineering effort is non-trivial, many capabilities are only supported for some variational objectives and not others. For example, as of this writing, Pyro's \texttt{ReweightedWakeSleep} objective~\cite{le_revisiting_2019} does not support minibatching, even though similar logic has already been implemented in other particle-based objectives. As another example, Pyro implements variance reduction strategies such as data-dependent baselines and enumeration of finite-support latent variables, but only for the standard ELBO variational objective; they have not yet been implemented for, e.g., the importance-weighted ELBO objective.
\item \textbf{Difficulty of reasoning.} The monolithic implementations of each variational objective's gradient estimation logic intertwine various concerns, including log density accumulation, automatic differentiation, gradient propagation through stochastic choices, and variance reduction logic. This can make it difficult to reason about correctness. Indeed, while the community has made tremendous progress in understanding the compositional correctness arguments of an increasingly broad class of Monte Carlo inference methods %\footnote{Monte Carlo methods are another approach to approximating intractable distributions, such as the posteriors of probabilistic inference problems.} 
for probabilistic programs~\cite{scibior_denotational_2017,scibior_functional_2018,lew_probabilistic_2023,lunden2021correctness,borgstrom2016lambda}, pioneering work on correctness for variational inference~\cite{lee_towards_2019,lee_smoothness_2023,li2023type} has generally focused on specific properties (e.g., smoothness and absolute continuity) in somewhat restricted languages, and not to end-to-end correctness of gradient estimation for variational inference. 
\end{itemize}

% Probabilistic programming languages (PPLs) with support for variational inference\textemdash for example, Pyro \cite{bingham_pyro_2018}, ProbTorch \cite{stites_learning_2021}, and Gen \cite{cusumano-towner_gen_2019}\textemdash go a long way to addressing these challenges. Users can implement variational families as probabilistic programs, and choose from a menu of automated variational inference algorithms to run. But each option on this menu monolithically combines a pre-set objective function $F$ and a pre-set gradient estimation strategy for that objective. Furthermore, some options only work on probabilistic programs that satisfy certain requirements, which are not always clearly documented. Applying an unsupported method may lead to runtime errors at best, or silent optimization failures at worst. For example, in Pyro, optimizing the reweighted wake-sleep (RWS) objective~\cite{le_revisiting_2019} fails silently if minibatching is enabled; as another example, using the \texttt{TraceEnum\_ELBO} algorithm on the Attend-Infer-Repeat model from Pyro's tutorials~\cite{eslami_attend_2016} raises an error (``Enumeration over cartesian product is not implemented''). One way of understanding these issues is that they arise from a lack of modularity in the implementation. In principle there is no reason that RWS should be incompatible with minibatching, or that enumeration should be incompatible with Attend-Infer-Repeat. Similarly, there is no reason that features like enumeration (supported only by \texttt{TraceEnum\_ELBO}), data-dependent baselines (supported only by \texttt{TraceGraph\_ELBO}), and importance-weighted objectives (supported only by \texttt{RenyiELBO}) should not be intercompatible. But because each objective function and gradient estimator must be implemented separately in its own algorithm, supporting every combination of features (carefully considering their interactions with each other and with various properties of the user's probabilistic program) is a Herculean task.\\ %For the same reason, it is difficult for users to extend today's PPLs to support new variational objective functions or gradient estimation strategies, as it requires expert knowledge not just of the relevant math but also of the PPL backend.\\

% Extending today's PPLs to support new variational objective functions or gradient estimation strategies is especially difficult, requiring expert knowledge not just of the relevant math but also of the PPL backend. Unlike Monte Carlo inference engines, which often have modular implementations and compositional correctness arguments~\cite{scibior_denotational_2017,scibior_functional_2018,lew2019trace}, PPL automation for VI is typically not implemented modularly, and to date there has been little attempt to formally characterize correctness guarantees of various components, and how they compose. %TODO: fix last sentence
% Finally, the probabilistic languages for defining variational families are generally not as expressive as state-of-the-art languages for Monte Carlo models and proposals~\cite{lew_probabilistic_2023}, lacking, e.g., support for general marginalization constructs or nested inference. These limitations motivate revisiting variational inference for probabilistic programs.
% \\\vspace{-2mm}

% Key ideas: 
% existing implementations of variational inference lack modularity: monolithic routines for 
% computing gradient estimates for training. 

% Variational inference (VI) is an important part of the modeling and inference toolkit. Probabilistic programming languages (PPLs) have been instrumental in making advanced VI techniques easier to use, enabling a wider array of practitioners to employ these methods within their models. But compared with the support PPLs afford for advanced Monte Carlo methods, PPL support for VI But the support for VI within PPLs has not kept pace with the developments for Monte Carlo (MC) inference methods.

% MC inference has benefitted from cutting-edge advancements, offering a high degree of modularity and programmability that unlocks a granular level of control. Practitioners enjoy the liberty to tailor proposal distributions, density estimation strategies, and particle evolutions, leveraging the full prowess of a programming language to customize each element. In stark contrast, the implementation of VI in PPLs like Pyro is restricted to a predefined selection of variational objectives and gradient estimation strategies, limiting the potential for customization and innovation.

% A closer examination reveals that both Monte Carlo proposals and VI variational families—known as guides in the world of PPLs—are authorable through user-defined programs. Yet, the languages employed to define these guides lack the expressive range found in the most advanced languages tailored for MC inference. This shortfall manifests in their inability to support operations such as marginalization and normalization, which are vital for the flexibility and expressiveness of probabilistic models.

% Furthermore, MC inference has been the subject of extensive semantic exploration, offering comprehensive frameworks that interpret the entire process of transforming user-written code into accurate implementations of inference algorithms. These frameworks involve a series of compositional steps that ensure the correctness and rigor of the underpinning methodology. Such cohesive semantic accounts are conspicuously absent for VI. This deficiency is reflected in the implementations of VI, where multiple concerns are enmeshed within the codebase, attempting to simultaneously manage density function computations, derivative calculations of deterministic functions, and the execution of Monte Carlo gradient estimation techniques.

% Probabilistic programming languages provide useful automation for modeling and inference. The automation which these systems provide can often save model and inference developers countless hours debugging their applications. To support a programmer interaction model which facilitates sound and correct inference, these systems typically expose interfaces for implementing inference algorithms - and formal guarantees that the inference quantities (e.g. Metropolis-Hastings accept reject ratios, or importance weights) computed by the interfaces are correct, and can be used to construct sound implementations of inference. Existing systems comfortably support the development of impressive applications, including automated data cleaning via user-programmable probabilistic heuristics \cite{lew_pclean_2021}, time series structure discovery and learning \cite{saad_bayesian_2019}, inverse graphics using rendering in the likelihood \cite{gothoskar_3dp3_2021}, and agent goal inference using probabilistic programs with planning algorithms \cite{zhi-xuan_online_2020}. The inference techniques utilized by these developments are fundamentally based on Monte Carlo inference methods. These methods have a long history of correctness guarantees, and recent work has extended these guarantees to expressive higher-order PPLs. 

% In contrast to Monte Carlo inference methods, variational inference has received less formal attention, yet variational inference has attractive runtime scaling properties, and is well suited to take advantage of data at scale \cite{ranganath_black_2014}. If practitioners seek to soundly integrate \textit{learnable} probabilistic programs into their modeling and inference stacks via variational inference, modern PPLs provide few guarantees. To provide automation and correctness guarantees for gradient estimators for variational objectives, PPL developers are faced with a difficult challenge: they must reason about the semantics of density computation and automatic differentiation \textit{together}. To avoid confronting this challenge head on, existing PPLs often choose to expose restricted gradient interfaces or black box variational objectives, without soundness guarantees or formalization. Practically, the ramifications of ignoring the formalism can be serious: when users utilize these interfaces - but choose to violate the assumptions of the system, existing systems will typically return silently incorrect results.
%\\\vspace{-1mm}

\paragraph{This work.} In this paper, we present a highly modular, highly programmable approach to supporting variational inference in PPLs. In our approach, all three ingredients of the variational inference problem\textemdash $\mathcal{P}$, $\mathcal{Q}$, and $\mathcal{F}$\textemdash are encoded as programs in expressive probabilistic languages, which support compositional annotation for specifying the desired mix of gradient estimation strategies. We then use a sequence of modular program transformations\textemdash each of which we independently prove correct\textemdash to construct unbiased gradient estimators for the user's variational objective.%\\\vspace{-1mm}%\footnote{A critical element to making this work is the recently introduced ADEV framework for modular gradient estimation~\cite{lew_adev_2023}: we specialize and extend ADEV to the variational inference setting. Our extensions include new constructs for differentiably tracing and estimating the densities of models and variational families (crucial for expressing virtually all variational objectives), a \textit{reverse-mode} ADEV implementation that efficiently computes gradient estimates in one pass (instead of one pass per parameter), and the first GPU-accelerated implementation of ADEV-style AD.}  %A particularly important extension  \textit{densities} of probabilistic programs, required by virtually all variational objectives. ADEV works in \textit{forward-mode}, and thus is hopelessly inefficient for optimizing neural networks with many parameters. I, and variational objectives $\mathcal{F}$ are typically expressed as functions of both expected values and density functions. The ADEV algorithm is a \textit{forward-mode} 

% \begin{itemize}[leftmargin=*]
% \item As in existing PPLs, users define variational families as probabilistic programs (\S\ref{sec:gen-transformations}). In \S\ref{sec:sp}, we extend our modeling language with constructs for marginalization and nested inference, bringing it to feature parity with state-of-the-art Monte Carlo PPLs~\cite{lew_probabilistic_2023}, and enabling users to express a broader class of variational families, e.g. that rely on auxiliary variables not present in the model. 
% \item Users define variational objectives in an expressive differentiable programming language based on ADEV~\cite{lew_adev_2023}. We extend ADEV to include primitives for simulating traces of, and computing or estimating densities of, models and variational families expressed as probabilistic programs. This enables a concise (4-line) implementation of common objectives like the ELBO, but also of many other objectives, like the importance-weighted ELBO~\cite{burda_importance_2016}, the reweighted wake-sleep objective~\cite{le_revisiting_2019}, hierarchical variational objectives~\cite{ranganath_hierarchical_2016}, and more.
% \item The gradient estimation strategy can be customized on a per-primitive basis when defining the variational family. Not every strategy can be applied in every context, but key conditions necessary for soundness are automatically enforced by the type system. These estimator annotations are automatically respected by the new ADEV constructs for working with probabilistic programs. 
% \end{itemize}


% We present a new design for a probabilistic programming language which supports the composition of unbiased gradient estimation and density computation to enable modular, correct by construction, variational inference. Our approach is based on a synthesis of ideas from existing formalized systems: we combine insights from the approach of \cite{lew_probabilistic_2023} to support a higher-order probabilistic programming language with \textbf{marginal} as a first-class construct, with gradient automation supported by using \cite{lew_adev_2023} as the target language of our program transformations. \\\vspace{-1mm}


\paragraph{Contributions.} This paper contributes:
\begin{itemize}[leftmargin=*]
    \item \textbf{Languages for models, variational families, and variational objectives}: We present an expressive language for models and variational families (\S\ref{sec:gen-lang}), similar to Gen, ProbTorch, or Pyro, along with an expressive differentiable language for variational objective functions (\S\ref{sec:adev-lang}).%, but with support for compositional annotation of gradient estimation strategies.
    %\item \textbf{Objective language}: In contrast to the menu-based approach of existing PPLs, we present an expressive differentiable language for variational objectives (\S\ref{sec:adev-lang}), by extending ADEV~\cite{lew_adev_2023} with constructs for tracing and estimating densities of probabilistic programs (\S\ref{sec:gen-transformations}).
    %\item \textbf{Modular design}: 
    \item \textbf{Flexible, modular automation}: We automate a broad class of unbiased gradient estimators for variational objectives (\S\ref{sec:adev}). New primitive gradient estimation strategies can be added modularly with just a few lines of code, without deeply understanding system internals (Appx.~\ref{appdx:extensibility}).
    \item \textbf{Formalization}: We formalize our approach as a sequence of composable program transformations (\S\ref{sec:gen-transformations}-\ref{sec:vi}) of simply-typed $\lambda$-calculi for probabilistic programs (\S\ref{sec:syntax}), and prove the unbiasedness of gradient estimation (under mild technical conditions) by logical relations (\S\ref{sec:correctness}). Ours is the first formal account of variational inference for PPLs that accounts for the interactions between tracing, density computation, gradient estimation strategies, and automatic differentiation.
    \item \textbf{System}: We contribute \texttt{genjax.vi}, a performant, GPU-accelerated implementation of our approach in JAX~\cite{frostig2018compiling}, which also extends our formal modeling language with constructs for marginalization and normalization (\S\ref{sec:sp})~\cite{lew_probabilistic_2023}. We also contribute concise, pedagogical Haskell and Julia versions. Our implementations are the first to feature \textit{reverse-mode} variants of the ADEV algorithm for modularly differentiating higher-order probabilistic programs~\cite{lew_adev_2023}.
    \item \textbf{Empirical evaluation}: We evaluate \texttt{genjax.vi} on several benchmark tasks, including inference in the challenging Attend-Infer-Repeat model~\cite{eslami_attend_2016}. Our evaluation shows that \texttt{genjax.vi} makes it possible to encode new gradient estimators that converge faster and to better solutions than Pyro's estimators. It also demonstrates, for the first time, that a version of ADEV can be scalably and performantly implemented, to deliver competitive performance on realistic probabilistic deep learning workloads.\footnote{\citet{lew_adev_2023} present only a toy Haskell implementation of  forward-mode ADEV, and report no experiments.}
\end{itemize}

Programmable inference \cite{mansinghka2018probabilistic} has often been understood as less automated but more powerful than generic inference. We emphasize that this paper \textit{expands} the automation provided by the system, relative to existing VI support in PPLs. This paper’s approach can automate the necessary gradient estimators for {arbitrary objectives} specified as programs (rather than the handful supported by existing PPLs), and can automatically use a combinatorial space of gradient estimation strategies, specified using compositional annotations on generative programs. %In \S\ref{sec:evaluation}, we show that the expanded class of gradient estimators that our system automates can out-perform standard estimators supported by existing systems.

% \noindent \textbf{Contributions.} This paper contributes:
% \begin{itemize}[leftmargin=*]
%     \item The first formalization for variational inference in a higher order probabilistic language, including \textit{compositional correctness guarantees} covering usage of a wide variety of variational objectives and gradient estimator strategies. 
%     \item Our language design exposes automation for \textit{expressive} variational objectives, including those defined by utilizing \textbf{marginal} to construct marginal distributions.
%     \item An \textbf{evaluation of our approach} on a set of case studies designed to test the performance and expressivity implications of our design. We establish several properties of our design: the overhead which our approach incurs compared to hand coded estimators is negligible, and our performance comparisons with well-supported variational inference PPLs are highly competitive. Our design also supports variational objectives which are not currently supported by any PPL - without losing in runtime cost.
% \end{itemize}

==> fig/adevjax/macros.tex <==
\newcommand{\KK}{\kappa}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\grad}{\nabla} 
\newcommand{\term}[0]{\star}
\newcommand{\ini}[0]{0}
\newcommand{\catC}{\mathbf{C}}
\newcommand{\catD}{\mathbf{D}}
\newcommand{\Set}[0]{\mathbf{Set}}
\newcommand{\SubSet}[0]{\mathbf{SubSet}}
\newcommand{\QBS}[0]{\mathbf{QBS}}
\newcommand{\Pred}[0]{\mathbf{Pred}}
\newcommand{\topo}[0]{\mathcal{J}}
\newcommand{\Cartsp}{\mathbf{CartSp}}
\newcommand{\Open}{\mathbf{Open}}
\newcommand{\plots}[0]{\mathcal{P}}
\newcommand{\conc}[1]{|#1|}
\newcommand{\wcpo}[0]{\ensuremath{\omega}cpo}
\newcommand{\wconc}[1]{\ensuremath{\conc{#1}_{\wcpo{}}}}
\newcommand{\site}[0]{(\catC,\topo)}
\newcommand{\concsh}[0]{Conc(\catC,\topo)}
\newcommand{\wconcsh}[0]{\omega\concsh}
\newcommand{\monos}[0]{\mathcal{M}}
\newcommand{\sitewmono}[0]{(\catC,\topo, \monos)}
\newcommand{\vcomp}[0]{\vdash^c}
\newcommand{\vval}[0]{\vdash^v}
\newcommand{\ter}[0]{t}
\newcommand{\val}[0]{v}
\newcommand{\sem}[1]{\llbracket #1\rrbracket}
\newcommand{\type}[0]{\tau}
\newcommand{\disctype}[0]{K}
\newcommand{\var}[0]{x}
\newcommand{\submono}[0]{Sub_\monos}
\newcommand{\cinf}[0]{c_\infty}
\newcommand{\mono}[0]{\rightarrowtail}
\newcommand{\vertn}[0]{\mathbb{V}_0}
\newcommand{\topovert}[0]{\mathcal{J}_V}
\newcommand{\shwvert}[0]{Sh(\catC+\vertn,\topo+\topovert)}
\newcommand{\monosv}[0]{\monos_V}
\newcommand{\wpap}[0]{\ensuremath{\omega}PAP}
\newcommand{\pap}[0]{PAP}
\newcommand{\topopap}[0]{\topo_{\pap}}
\newcommand{\monopap}[0]{\monos_{\pap}}
\newcommand{\cpap}[0]{c\pap}
\newcommand{\crepr}[0]{\mathbf{c-Repr}}
\newcommand{\pcfv}[0]{PCF\ensuremath{_V}}
\newcommand{\iso}[0]{\cong}
\newcommand{\cst}[0]{\underline{c}}
\newcommand{\pRR}[0]{\mathbb{W}}
\newcommand{\contm}[0]{\mathcal{J}}
\newcommand{\bind}[0]{\mathop{\gg\mkern-10mu\scalebox{1}[1]{=}}}
\newcommand{\iterate}[0]{\texttt{iterate}}
\newcommand{\ebind}[0]{>\mkern-5mu=\mkern-5mu>}
\newcommand{\monstruct}[0]{(T, \return, \bind)}
\newcommand{\epic}[0]{\twoheadrightarrow}
\newcommand{\randm}[0]{R}
\newcommand{\expect}[0]{\mathbb{E}}
\newcommand{\lift}[0]{\mathbf{L}}
\newcommand{\wclos}[0]{Cl_{\omega}}
\newcommand{\shclos}[0]{Cl_{sh}}
\newcommand{\shwclos}[0]{Cl_{\omega sh}}
\newcommand{\varm}[0]{\mathbb{V}}
\newcommand{\seeds}[0]{\Omega}
\newcommand{\dom}[0]{Dom}
\newcommand{\measm}[0]{T}
\newcommand{\measmm}[0]{T2}
\newcommand{\lub}[0]{\bigvee}
\newcommand{\setprim}[0]{\mathcal{F}}
\newcommand{\lang}[0]{\mathcal{L}}
\newcommand{\elang}[0]{\mathcal{L}_\mathcal{P}}
\newcommand{\manif}[0]{\mathcal{M}}
\newcommand{\tangent}[0]{\mathcal{T}}
\newcommand{\hausd}[0]{\mathcal{H}}
\newcommand{\eqwsh}[0]{\mathcal{E}_{\omega,sh}}
\newcommand{\omsh}[0]{\omega sheaves}
\newcommand{\modwsh}[0]{Mod(\omsh,\Set)}
\newcommand{\op}[0]{op}
\newcommand{\ops}[0]{Op}
\newcommand{\pop}[1]{\ensuremath{\partial_i}\op}
\newcommand{\context}[0]{\Gamma}
\newcommand{\adsymbol}[0]{\ensuremath{\mathcal{D}}}
\newcommand{\ad}[1]{\ensuremath{\mathcal{D}\{#1\}}}
\newcommand{\verifsymbol}[0]{\ensuremath{\mathcal{V}}}
\newcommand{\verif}[1]{\ensuremath{\mathcal{V}\{#1\}}}
\newcommand{\computations}[0]{\mathcal{V}}
\newcommand{\values}[0]{\mathcal{V}}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\syntaxcolor}[0]{\color{blue!70!black}}
\newcommand{\constantcolor}[1]{\mathbf{\syntaxcolor{#1}}}
\newcommand{\colforsyntax}[1]{\mathbf{\syntaxcolor{#1}}}
\newcommand{\eqbe}[0]{\stackrel{\beta\eta}{=}}
\newcommand{\inl}[0]{\colforsyntax{inl}}
\newcommand{\inr}[0]{\colforsyntax{inr}}
\newcommand{\case}[0]{\colforsyntax{case}}
\newcommand{\True}[0]{\colforsyntax{True}}
\newcommand{\False}[0]{\colforsyntax{False}}
\newcommand{\coupled}[0]{\colforsyntax{coupled}}
\newcommand{\haskdo}[0]{\colforsyntax{do}}
\newcommand{\dhaskdo}[0]{\colforsyntax{do}_\mathcal{D}}
\newcommand{\of}[0]{\colforsyntax{of}}
\newcommand{\iiflet}[0]{\colforsyntax{if}}
\newcommand{\llet}[0]{\colforsyntax{let}}
\newcommand{\iin}[0]{\colforsyntax{in}}
\newcommand{\iif}[0]{\colforsyntax{if}}
\newcommand{\then}[0]{\colforsyntax{then}}
\newcommand{\eelse}[0]{\colforsyntax{else}}
\newcommand{\iifthenelse}[3]{\iif~#1~\then~#2~\eelse~#3}
\newcommand{\return}[0]{\colforsyntax{return}}
\newcommand{\dup}[0]{\texttt{dup}}
\newcommand{\drop}[0]{\texttt{drop}}
\newcommand{\dreturn}[0]{\colforsyntax{return}_\mathcal{D}}
\newcommand{\vreturn}[0]{\return_\ver}
\newcommand{\vhaskdo}[0]{\haskdo_\ver}
\newcommand{\fst}[0]{\colforsyntax{fst}}
\newcommand{\snd}[0]{\colforsyntax{snd}}
\newcommand{\splits}[0]{\mathbf{split}}
\newcommand{\logs}{\texttt{log}}
\newcommand{\exps}{\texttt{exp}}
\newcommand{\sins}{\texttt{sin}}
\newcommand{\coss}{\texttt{cos}}
\newcommand{\pows}{\texttt{pow}}
\newcommand{\der}{\mathcal{D}}
\newcommand{\ver}{\mathcal{V}}
\newcommand{\typecolor}[1]{\mathbf{\syntaxcolor{#1}}}
\newcommand{\Real}[0]{\typecolor{Real}}
\newcommand{\Float}[0]{\typecolor{Float}}
\newcommand{\Dual}[0]{\typecolor{Dual}}
\newcommand{\data}[0]{\typecolor{data}}
\newcommand{\sample}[0]{\constantcolor{uniform}}
\newcommand{\normalreparam}[0]{\constantcolor{normal_\texttt{REPARAM}}}
\newcommand{\normalreinforce}[0]{\constantcolor{normal_\texttt{REINFORCE}}}
\newcommand{\geometricreinforce}[0]{\constantcolor{geometric_\texttt{REINFORCE}}}
\newcommand{\flipreinforce}[0]{\constantcolor{flip_\texttt{REINFORCE}}}
\newcommand{\flipenum}[0]{\constantcolor{flip_\texttt{ENUM}}}
\newcommand{\score}[0]{\constantcolor{score}}
\newcommand{\gammareparam}[0]{\constantcolor{gamma_\texttt{REPARAM}}}
\newcommand{\studenttreparam}[0]{\constantcolor{student\_t_\texttt{REPARAM}}}
\newcommand{\betareparam}[0]{\constantcolor{beta_\texttt{REPARAM}}}
\newcommand{\dirichletreparam}[0]{\constantcolor{dirichlet_\texttt{REPARAM}}}
\newcommand{\baseline}[0]{\constantcolor{baseline}}
\newcommand{\flipimportance}[0]{\constantcolor{flip_\texttt{IMPORTANCE}}}
\newcommand{\addcost}[0]{\constantcolor{add\_cost}}
\newcommand{\poissonweak}[0]{\constantcolor{poisson_\texttt{WEAK\_DERIV}}}
\newcommand{\gammaimplicit}[0]{\constantcolor{gamma_\texttt{IMPLICIT}}}
\newcommand{\importance}[0]{\constantcolor{importance}}
\newcommand{\reinforce}[0]{\constantcolor{reinforce}}
\newcommand{\leaveoneout}[0]{\constantcolor{leave\_one\_out}}
\newcommand{\smc}[0]{\constantcolor{smc}}
\newcommand{\implicitdiff}[0]{\constantcolor{implicit\_differentiation}}
\newcommand{\reparamreject}[0]{\constantcolor{reparam\_rejection\_sampler}}
\newcommand{\forget}[1]{\lfloor #1 \rfloor}
\newcommand{\types}[0]{Types}
\newcommand{\catV}[0]{\mathbf{V}}
\newcommand{\kleisli}[0]{\mathbf{Kleisli}}
\newcommand{\paral}{\mathbin{\!/\mkern-5mu/\!}}
\newcommand{\fib}[3]{#1:\mathbb{#2}\to\mathbb{#3}}
\newcommand{\mbe}{\constantcolor{\mathbb{E}}}
\newcommand{\mbb}{\mathbb{B}}
\newcommand{\mba}{\mathbb{A}}
\newcommand{\mbc}{\mathbb{C}}
\newcommand{\mbd}{\mathbb{D}}
\newcommand{\mbl}{\mathbb{L}}
\newcommand{\eRR}{\widetilde{\RR}}
\newcommand{\deRR}{\eRR_\mathcal{D}}
\newcommand{\posreal}[0]{\RR_{> 0}}
\newcommand{\eplus}{+^{\eRR}}
\newcommand{\etimes}{\times^{\eRR}}
\newcommand{\eexp}{exp^{\eRR}}
\newcommand{\minibatch}{\constantcolor{minibatch}}
\newcommand{\exact}{\constantcolor{exact}}
\newcommand{\monadsymbol}{P}
\newcommand{\pmonad}{\monadsymbol\,}
\newcommand{\dpmonad}{\monadsymbol_\der\,}
\newcommand{\vpmonad}{\monadsymbol_\ver\,}
\newcommand{\rel}{\mathscr{R}}
\newcommand{\arr}[1]{#1^{\to}}
\newcommand{\pushoutcorner}[1][dr]{\save*!/#1+1.2pc/#1:(1,-1)@^{|-}\restore}
\newcommand{\pullbackcorner}[1][dr]{\save*!/#1-1.2pc/#1:(-1,1)@^{|-}\restore}
\newcommand{\lcstruct}[0]{\lambda_c(\Sigma)}
\newcommand{\lifted}[0]{\stackrel{\cdot}{\to}}
\newcommand{\Gl}[0]{\mathbf{Gl}}
\newcommand{\semgl}[1]{\llparenthesis #1\rrparenthesis}
\newcommand{\facto}[0]{\ensuremath{(\mathcal{E},\mathcal{M})}}
\newcommand{\qbd}{\mathbf{Qbd}}
\newcommand{\bdiff}{\mathbf{BDiff}}

==> fig/air_comparisons/accuracy_elbo_wall_clock_time.tex <==
\begin{figure}[htb!]
\includegraphics[width=\textwidth]{fig/air_comparisons/accuracy_elbo_wall_clock_time.pdf}
\caption{AIR training comparisons (top: accuracy, bottom: objective value, vs. wall clock time) between \texttt{genjax.vi} and Pyro. We evaluate a variety of custom estimators and objectives (ELBO, IWELBO) using our system, several of which are not expressible in Pyro, or come with serious limitations (like mini-batching disallowed). Our implementation supports drastically faster convergence in wall clock time (seconds, versus minutes), even for estimators which include enumeration or involve running importance sampling (IWELBO). Compared to Pyro's recommended estimator (REINFORCE + neural baselines), our best estimator (IWAE + MVD, not expressible in Pyro) converges an order of magnitude faster.}
\label{fig:elbo_acc_clock}
\end{figure}

==> fig/example_transcript/expressive_variational.tex <==
\begin{minted}[numbersep=5pt,baselinestretch=1.0, escapeinside=||,mathescape=true,linenos]{haskell}
|$\textcolor{gray}{\textit{# Hierarchical variational family with latent variable v}}$|
guide_joint |$\texttt{:}$| |$\mathbb{R}^2$| |$\rightarrow$| |$\texttt{\textbf{G}}$| |$\mathbb{R}^2$|
guide_joint |$\texttt{=}$| |$\lambda \phi$|. |$\texttt{\textbf{do}}$|
  v |$\leftarrow$| |\textbf{sample}| |$\texttt{uniform}$|(0.0, 2|$\pi$|) "v"
  |$\textbf{\texttt{let}}$| (|$\log\sigma_1$|, |$\log\sigma_2$|) |$\texttt{=}$| |$\phi$|
  x |$\leftarrow$| |\textbf{sample}| |$\texttt{normal}_\text{REPARAM}$|(sqrt(5.0) * cos(v), |$e^{\log\sigma_1}$|) "x"
  y |$\leftarrow$| |\textbf{sample}| |$\texttt{normal}_\text{REPARAM}$|(sqrt(5.0) * sin(v), |$e^{\log\sigma_2}$|) "y"
  |\textbf{return}| (x, y)
|$\textcolor{gray}{\textit{# Marginalize the auxiliary variable with 5-particle IS}}$|
marginal_guide |$\texttt{:}$| |$\mathbb{R}^2$| |$\rightarrow$| |$\texttt{\textbf{G}}$| |$\mathbb{R}^2$|
marginal_guide |$\texttt{=}$| |$\lambda \phi.\texttt{\textbf{marginal}}$| ["x","y"] (guide_joint |$\phi$|) 
          (|$\lambda \_. {\textbf{\texttt{importance}}}$| (|\textbf{sample}| |$\texttt{uniform}$|(0, 2|$\pi$|) "v") 5)
\end{minted}

==> fig/example_transcript/model_prior.tex <==
\begin{minted}[numbersep=5pt,baselinestretch=1.0,escapeinside=||,mathescape=true,linenos]{haskell}
|$\textcolor{gray}{\textit{# Model: (x,y) latent, z observed to equal 5.0}}$|
model |$\texttt{:}$| |$\texttt{\textbf{G}}$| |$\mathbb{R}^2$|
model |$\texttt{=}$| |$\texttt{\textbf{do}}$|
  x |$\leftarrow$| |\textbf{sample}| |$\texttt{normal}_\text{REPARAM}$|(0.0, 10.0) "x"
  y |$\leftarrow$| |\textbf{sample}| |$\texttt{normal}_\text{REPARAM}$|(0.0, 10.0) "y"
  |$\texttt{\textbf{let}}$| r |$\texttt{=}$| x|$^2$| + y|$^2$|
  |$\texttt{\textbf{let}}$| |$\sigma$| |$\texttt{=}$| 0.1 + (r / 100.0)
  |$\texttt{\textbf{observe}}$| |$\texttt{normal}_\text{REPARAM}$|(r, |$\sigma$|) 5.0 |$\textcolor{gray}{\textit{# z}}$|
  |\textbf{return}| (x, y)
\end{minted}

==> fig/example_transcript/naive_variational.tex <==
\begin{minted}[numbersep=5pt,baselinestretch=1.0,escapeinside=||,mathescape=true,linenos]{haskell}
|$\textcolor{gray}{\textit{# Variational family with parameters $\phi$}}$|
naive_guide |$\texttt{:}$| |$\mathbb{R}^4$| |$\rightarrow$| |$\texttt{\textbf{G}}$| |$\mathbb{R}^2$|
naive_guide |$\texttt{=}$| |$\lambda\phi$|. |$\texttt{\textbf{do}}$|
  |$\textbf{\texttt{let}}$| (|$\mu_1$|, |$\mu_2$|, |$\log\sigma_1$|, |$\log\sigma_2$|) |$\texttt{=}$| |$\phi$|
  x |$\leftarrow$| |\textbf{sample}| |$\texttt{normal}_\text{REPARAM}$|(|$\mu_1$|, |$e^{\log\sigma_1}$|) "x"
  y |$\leftarrow$| |\textbf{sample}| |$\texttt{normal}_\text{REPARAM}$|(|$\mu_2$|, |$e^{\log\sigma_2}$|) "y"
  |\textbf{return}| (x, y)
\end{minted}

==> fig/example_transcript/sir_guide.tex <==
\begin{minted}[numbersep=5pt,baselinestretch=1.0,escapeinside=||,mathescape=true,linenos]{haskell}
|$\textcolor{gray}{\textit{# N-particle IS as variational family}}$|
sir_guide |$\texttt{:}$| |$\mathbb{R}^4$| |$\rightarrow$| |$\texttt{\textbf{G}}$| |$\mathbb{R}^2$|
sir_guide |$\texttt{=}$| |$\lambda\phi$|.
  |$\textbf{\texttt{normalize}}$| model
  (|$\textbf{\texttt{importance}}$|
   (naive_guide |$\phi$|)
   |$\texttt{N}$|)
\end{minted}

==> fig/example_transcript/transcript.tex <==
\begin{figure}
\vspace{-5mm}
\centering
% Row 1: Code on the left, Image on the right
\hfill
\begin{minipage}{0.43\textwidth}
\input{fig/example_transcript/model_prior}
\end{minipage}
\hfill
\hfill
\hfill
\begin{minipage}{0.43\textwidth}
\centering
\includegraphics[width=0.8\linewidth]{fig/example_transcript/fig_2_model_prior.pdf}
\end{minipage}
\vspace{-3mm}
\hrule
\vspace{0.1cm} % Adds vertical space after the line
% Row 2: Code on the left, Image on the right
\hfill
\begin{minipage}{0.43\textwidth}
\input{fig/example_transcript/naive_variational}
\end{minipage}
\hfill
\hfill
\hfill
\begin{minipage}{0.43\textwidth}
\centering
{\footnotesize\textbf{Trained variational approximation (ELBO)}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{c c}
\includegraphics[width=0.45\linewidth]{fig/example_transcript/fig_2_naive_variational_elbo_samples.pdf} & \includegraphics[width=0.45\linewidth]{fig/example_transcript/fig_2_naive_variational_elbo_samples_2.pdf}
\end{tabular}
}
\end{minipage}
\vspace{0.1cm} % Adds vertical space after the line
\hrule
\vspace{0.1cm} % Adds vertical space after the line
% Row 3: Code on the left, Image on the right
\hfill
\begin{minipage}{0.3\textwidth}
\input{fig/example_transcript/sir_guide}
\end{minipage}%
\hfill
\hfill
\begin{minipage}{0.60\textwidth}
\centering
{\scriptsize\setlength{\tabcolsep}{-0.1mm}
\begin{tabular}{c c c c}
\multicolumn{3}{c}{\makecell{\textbf{Trained} \texttt{naive\_guide} \textbf{using IWELBO($N$)}}} & \makecell{\tiny{\textbf{Trained} \texttt{sir\_guide}} \\ \tiny{\textbf{with $N = 30$}}} \\
\includegraphics[width=0.23\linewidth]{fig/example_transcript/fig_2_naive_variational_iwae_elbo_10_samples.pdf} & \includegraphics[width=0.23\linewidth]{fig/example_transcript/fig_2_naive_variational_iwae_elbo_20_samples.pdf} & \includegraphics[width=0.23\linewidth]{fig/example_transcript/fig_2_naive_variational_iwae_elbo_30_samples.pdf} &
\includegraphics[width=0.23\linewidth]{fig/example_transcript/fig_2_naive_variational_iwae_elbo_30_sir_samples.pdf} \\
\textbf{$N = 10$} & \textbf{$N = 20$} & \textbf{$N = 30$} &
\end{tabular}}
\end{minipage}
\vspace{0.1cm} % Adds vertical space after the line
\hrule
\vspace{0.1cm} % Adds vertical space after the line
% Row 4: Code on the left, Image on the right
\hfill
\begin{minipage}{0.7\textwidth}
\input{fig/example_transcript/expressive_variational}
\end{minipage}%
\hfill
\begin{minipage}{0.24\textwidth}
{\tiny
\begin{tabular}{c}
\textbf{Untrained} \\
\includegraphics[width=0.7\linewidth]{fig/example_transcript/fig_2_untrained_expressive_variational_elbo_samples.pdf} \\
\makecell{\textbf{Trained using HVI ELBO}} \\
\includegraphics[width=0.7\linewidth]{fig/example_transcript/fig_2_hvi_expressive_variational_elbo_samples.pdf}
\end{tabular}}
\end{minipage}
\Description{A transcript of using our framework.}
\caption{Designing variational inference algorithms to solve a posterior problem using our approach. (\textbf{Top}) A generative model of noisy samples near a cone, observing $z = 5$ induces a posterior problem: the true posterior is close to a circle with radius $r = \sqrt{5}$. (\textbf{Second}) A variational family using a pair of axis aligned normal distributions, with learnable means and standard deviations: ELBO optimization using this family results in an approximation which covers a small part of the true posterior. (\textbf{Third}) Practitioners may consider strategies to improve the guide: using $N$-particle sampling importance resampling with a custom proposal (\texttt{sir\_guide}) as the guide is equivalent to IWELBO optimization, increasing $N$ improves coverage. (\textbf{Final}) Another strategy: adding auxiliary latent variables and using marginalization (\texttt{marginal\_guide}) to define the guide is equivalent to HVI ELBO optimization. Both strategies improve the results: our approach automates unbiased gradient estimators for both, and many more.}
\label{fig:example_transcript}
\end{figure}

==> fig/expressivity_table/checks_exes_table.tex <==
\setlength{\dashlinedash}{0.2pt}
\setlength{\dashlinegap}{2pt}
\setlength{\arrayrulewidth}{0.2pt}


\begin{table}[h]
\centering
\caption{\label{tab:my_label}We consider a combinatorial space of gradient estimators and objective functions that can be optimized for the Attend-Infer-Repeat (AIR) model. Here, we focus on strategies for the discrete random choices and assume that multivariate normal choices use reparametrization. Pyro supports only a pre-selected menu of options within this combinatorial space, whereas \texttt{genjax.vi} can express them all, compositionally.}
\scriptsize{\begin{tabular}{|cccc|c|c|cc|}
\hline
\multicolumn{4}{|c|}{\textbf{Active Gradient Estimation Strategies}} & \multirow{2}{*}{\textbf{Objective}} & \multirow{2}{*}{\textbf{Batch Size}} & \multicolumn{2}{|c|}{\textbf{System}} \\
REINFORCE & ENUM & BASELINE & MVD &  &  & Pyro & Ours \\\hline
\multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{ } & \multirow{2}{*}{ } & \multirow{2}{*}{ } & ELBO & $\geq$ 1 & \textcolor{teal}{\textbf{$\checkmark$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
& & & & IWAE & $\geq$ 1 & \textcolor{teal}{\textbf{$\checkmark$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hdashline
\multirow{2}{*}{ } & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{ } & \multirow{2}{*}{ } & ELBO & $\geq$ 1 & \textcolor{teal}{\textbf{$\checkmark$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
& & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hdashline
\multirow{2}{*}{ } & \multirow{2}{*}{ } & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{ } & ELBO & $\geq$ 1 & \textcolor{teal}{\textbf{$\checkmark$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
& & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hdashline
\multirow{2}{*}{ } & \multirow{2}{*}{ } & \multirow{2}{*}{ } & \multirow{2}{*}{$\checkmark$} & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
& & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hdashline
\multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{ } & \multirow{2}{*}{ } & ELBO & $\geq$ 1 & \textcolor{teal}{\textbf{$\checkmark$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
& & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hdashline
\multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{ } & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{ } & ELBO & $\geq$ 1 & \textcolor{teal}{\textbf{$\checkmark$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
& & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hdashline
\multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{ } & \multirow{2}{*}{ } & \multirow{2}{*}{$\checkmark$} & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
& & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hdashline
\multirow{2}{*}{ } & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{ } & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
& & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hdashline
\multirow{2}{*}{ } & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{ } & \multirow{2}{*}{$\checkmark$} & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
& & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hdashline
\multirow{2}{*}{ } & \multirow{2}{*}{ } & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{$\checkmark$} & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
& & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hdashline
\multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{ } & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
& & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hdashline
\multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{ } & \multirow{2}{*}{$\checkmark$} & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
& & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hdashline
\multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{ } & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{$\checkmark$} & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
& & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hdashline
\multirow{2}{*}{ } & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{$\checkmark$} & \multirow{2}{*}{$\checkmark$} & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
& & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hdashline
\multicolumn{4}{|c|}{\multirow{2}{*}{Not Exploited}} & RWS & 1 & \textcolor{teal}{\textbf{$\checkmark$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\multicolumn{4}{|c|}{} & RWS & $>$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
\cdashline{5-8}
\hline
\end{tabular}}
\end{table}



% \begin{table}[h]
% \caption{\label{tab:my_label}We consider a combinatorial space of gradient estimators and objective functions that can be optimized for the Attend-Infer-Repeat (AIR) model. Here, we focus on strategies for the discrete random choices and assume that multivariate normal choices use reparametrization. Pyro supports only a pre-selected menu of options within this combinatorial space, whereas \texttt{genjax.vi} can express them all, compositionally.}
% \centering
% \footnotesize{\begin{tabular}{|cccc|c|c|cc|}
% \hline
% \multicolumn{4}{|c|}{\textbf{Active Gradient Estimation Strategies}} & \multirow{2}{*}{\textbf{Objective}} & \multirow{2}{*}{\textbf{Batch Size}} & \multicolumn{2}{|c|}{\textbf{System}} \\
% REINFORCE & ENUM & BASELINE & MVD &  &  & Pyro & Ours \\\hline
% \multirow{4}{*}{$\checkmark$} & \multirow{4}{*}{ } & \multirow{4}{*}{ } & \multirow{4}{*}{ } & ELBO & $\geq$ 1 & \textcolor{teal}{\textbf{$\checkmark$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & IWAE & $\geq$ 1 & \textcolor{teal}{\textbf{$\checkmark$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & 1 & \textcolor{teal}{\textbf{$\checkmark$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & > 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \hdashline
% \multirow{3}{*}{ } & \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{ } & \multirow{3}{*}{ } & ELBO & $\geq$ 1 & \textcolor{teal}{\textbf{$\checkmark$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \hdashline
% \multirow{3}{*}{ } & \multirow{3}{*}{ } & \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{ } & ELBO & $\geq$ 1 & \textcolor{teal}{\textbf{$\checkmark$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \hdashline
% \multirow{3}{*}{ } & \multirow{3}{*}{ } & \multirow{3}{*}{ } & \multirow{3}{*}{$\checkmark$} & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \hdashline
% \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{ } & \multirow{3}{*}{ } & ELBO & $\geq$ 1 & \textcolor{teal}{\textbf{$\checkmark$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \hdashline
% \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{ } & \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{ } & ELBO & $\geq$ 1 & \textcolor{teal}{\textbf{$\checkmark$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \hdashline
% \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{ } & \multirow{3}{*}{ } & \multirow{3}{*}{$\checkmark$} & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \hdashline
% \multirow{3}{*}{ } & \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{ } & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \hdashline
% \multirow{3}{*}{ } & \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{ } & \multirow{3}{*}{$\checkmark$} & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \hdashline
% \multirow{3}{*}{ } & \multirow{3}{*}{ } & \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{$\checkmark$} & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \hdashline
% \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{ } & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \hdashline
% \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{ } & \multirow{3}{*}{$\checkmark$} & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \hdashline
% \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{ } & \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{$\checkmark$} & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \hdashline
% \multirow{3}{*}{ } & \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{$\checkmark$} & \multirow{3}{*}{$\checkmark$} & ELBO & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & IWAE & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \cdashline{5-8}
% & & & & RWS & $\geq$ 1 & \textcolor{purple}{\textbf{$\times$}} & \textcolor{teal}{\textbf{$\checkmark$}} \\
% \hline
% \end{tabular}}
% \end{table}

==> fig/expressivity_table/expressivity_table.tex <==
\begin{figure}[htb!]
\centering
\begin{tabular}{ | c c | c | c | c | c | }
    \hline
    System & Compiler & AIR & AIR (enum) & IWAE AIR & IWAE AIR (enum) \\
    \hline
    \texttt{genjax.vi}    & JAX (XLA) & 1.52 $\pm$ 0.05 & 6.22 $\pm$ 0.29 & 2.28 $\pm$ 0.12 & 50.7 $\pm$ 1.2 \\
    \texttt{pyro}            & Torch & 72.2 & \text{\sffamily X} & 76.3 & \text{\sffamily X} \\
    \hline
\end{tabular}
\label{fig:expressivity_table}
\end{figure}

==> fig/overhead/code.tex <==
\begin{minted}[framesep=3mm, baselinestretch=1.0, escapeinside=||, mathescape=true, linenos]{python}
@genjax.gen
def model(decoder):
  latent = genjax.vi.mv_normal_diag_reparam(
    zeros(10), ones(10)
  ) @ "latent"
  logits = decoder(latent)
  genjax.vi.flip_reinforce(logits) @ "image"

@genjax.gen
def guide(encoder, chm):
    image = chm["image"]
    loc, scale_diag = encoder(image)
    genjax.vi.mv_normal_diag_repram(
      loc, scale_diag
    ) @ "latent"

chm = genjax.choice_map({"image": data})

@genjax.adev
def elbo(decoder, encoder):
    (v, w_q) = guide.sim(guide_args, chm)
    w_p = model.density(merge(v, chm), decoder)
    return log(w_p) - log(w_q)

key = PRNGKey(314159)
elbo.grad_estimate(key, (decoder, ), (encoder, chm))
\end{minted}

==> fig/sec3-adev-copy.tex <==
\begin{figure}[t]
\scriptsize{
\begin{tabular}{ll}
    % Overall spec
   {Spec}  & \framebox{\textcolor{blue}{\textbf{\textit{Syntax}}} \;\; $\vdash t : \RR^n \to \eRR \implies \vdash \mathbf{adev}\{t\} : \RR^n \to \RR^n \to \eRR$ \quad \;\textcolor{blue}{\textbf{\textit{Semantics}}} \;\; $\mathbb{E}_{x \sim \sem{\mathbf{adev}\{t\}}(\mathbf{\theta}, \mathbf{v})}[x] = \left(\nabla_\theta \int_{\RR} x~\sem{t}(\mathbf{\theta}, dx)\right)^T \mathbf{v}$} \\
   % Wrapper implementation
   \rule{0pt}{4ex}{Wrapper}  & $\mathbf{adev}\{t\} \coloneqq \lambda \theta. \lambda \mathbf{v}. \mathbb{E} (\haskdo \{(y, y') \gets \mathcal{D}\{t\}~((\theta_1, \mathbf{v}_1),\dots,(\theta_n, \mathbf{v_n})); \return~y'\})$\\
   % Spec for helper
   \rule{0pt}{6ex}{Helper} $\mathcal{D}$ & \framebox{\textcolor{blue}{\textbf{\textit{Syntax}}}\;\;$\Gamma \vdash_{\text{ADEV}} t : \tau \implies \mathcal{D}\{\Gamma\} \vdash_{\text{ADEV}} \mathcal{D}\{t\} : \mathcal{D}\{\tau\}$\quad \quad\textcolor{blue}{\textbf{\textit{Semantics}}}\;\;$\forall (\gamma, \gamma') \in R^{\mathcal{D}}_{\Gamma}, (\sem{t} \circ \gamma, \sem{\mathcal{D}\{t\}} \circ \gamma') \in R^{\mathcal{D}}_\tau$}\\
   % Implementation on types
    \rule{0pt}{4ex}\;\textit{on types} & \begin{tabular}[t]{@{}l@{}l|l@{}l}
        $\mathcal{D}\{\RR\}$ &$\coloneqq \RR \times \RR$ & $R^\mathcal{D}_\RR$ &$\coloneqq \{(f, g) \mid g = \lambda r. (f(r), f'(r))\}$\\
        $\mathcal{D}\{\sigma\}$ &$\coloneqq \sigma \quad\quad\quad (\sigma \in \{\RR^*, \mathbb{B}, \text{Str}\})$ & $R^\mathcal{D}_{\sigma}$ &$\coloneqq \{(f, f) \mid f\text{ constant}\}$\\
        $\mathcal{D}\{\tau_1 \times \tau_2\}$&$\coloneqq \mathcal{D}\{\tau_1\} \times \mathcal{D}\{\tau_2\}$ & $R^\mathcal{D}_{\tau_1 \times \tau_2}$ &$\coloneqq \{(f,g) \mid \forall i \in \{1, 2\}. (\pi_i \circ f, \pi_i \circ g) \in R^\mathcal{D}_{\tau_i}\}$\\
        $\mathcal{D}\{\tau_1 \to \tau_2\}$&$\coloneqq \mathcal{D}\{\tau_1\} \to \mathcal{D}\{\tau_2\}$ & $R^\mathcal{D}_{\tau_1 \to \tau_2}$ &$\coloneqq \{(f,g) \mid \forall (x,y) \in R^\mathcal{D}_{\tau_1}, (\lambda r. f(r)(x(r)),g(r)(y(r))) \in R^\mathcal{D}_{\tau_2}\}$\\
        % $\mathcal{D}\{\RR^*\}$ &$\coloneqq \RR^*$ & $R^\mathcal{D}_{\RR^*}$ &$\coloneqq \{(f, f) \mid f\text{ constant}\}$\\
        % $\mathcal{D}\{\mathbb{B}\}$ &$\coloneqq \mathbb{B}$ & $R^\mathcal{D}_\mathbb{B}$ &$\coloneqq \{(f, f) \mid f \text{ constant}\}$ \\
        % $\mathcal{D}\{\text{Str}\}$ &$\coloneqq \text{Str}$ & $R^\mathcal{D}_\text{Str}$ &$\coloneqq \{(f, f) \mid f \text{ constant}\}$ \\
        $\mathcal{D}\{\trace\}$ &$\coloneqq \trace$ & $R^\mathcal{D}_\trace$ &$\coloneqq \{(f, g) \mid \forall k \in \sem{\text{Str}}. (\lambda r. f(r)[k], \lambda r. g(r)[k]) \in R^{\mathcal{D}}_\sigma\}$ \\
        $\mathcal{D}\{D~\sigma\}$&$\coloneqq \mathcal{D}\{P~\sigma\}$ & $R^\mathcal{D}_{D~\sigma}$ &$\coloneqq R^\mathcal{D}_{P~\sigma}$\\
        $\mathcal{D}\{\eRR\}$&$\coloneqq P~(\RR \times \RR)$ & $R^\mathcal{D}_{\eRR}$ &$\coloneqq \{(\mu, \nu) \mid (\lambda r. \mathbb{E}_{x \sim \mu(r)}[x], \lambda r. (\mathbb{E}_{(x,y) \sim \nu(r)}[x], \mathbb{E}_{(x,y) \sim \nu(r)}[y])) \in R_\RR^\mathcal{D}\}$\\
        $\mathcal{D}\{P~\tau\}$&$\coloneqq (\mathcal{D}\{\tau\} \to \mathcal{D}\{\eRR\}) \to \mathcal{D}\{\eRR\}$ & $R^\mathcal{D}_{P~\tau}$ &$\coloneqq \{(\mu, \nu) \mid (\lambda r. \lambda k. \lambda U. \mathbb{E}_{x \sim \mu(r)}[k(x, U)], \nu) \in R^{\mathcal{D}}_{(\tau \to \eRR) \to \eRR} \}$
    \end{tabular} \\
   % \rule{0pt}{4ex}\quad\textit{on types} & $\xi\{\sigma\} \coloneqq \sigma \;\mid\; \xi\{D~\sigma\} \coloneqq \sigma \to \RR \;\mid\; \xi\{\tau_1 \to \tau_2\} \coloneqq \xi\{\tau_1\} \to \xi\{\tau_2\}$ \\
   % Implementation on terms
   \rule{0pt}{4ex}\;\textit{on terms} & \begin{tabular}[t]{@{}l@{}ll@{}l}
   $\mathcal{D}\{()\}$ &$\coloneqq ()$ &
   $\mathcal{D}\{\{\}\}$ &$\coloneqq \{\}$ \\
   $\mathcal{D}\{c\}$ &$\coloneqq c_\mathcal{D}$ &
   $\mathcal{D}\{x\}$ &$\coloneqq x$ \\
   $\mathcal{D}\{\lambda x. t\}$&$\coloneqq \lambda x. \mathcal{D}\{t\}$ &
   $\mathcal{D}\{t_1~t_2\}$&$\coloneqq \mathcal{D}\{t_1\}~\mathcal{D}\{t_2\}$ \\
   $\mathcal{D}\{(t_1,t_2)\}$&$\coloneqq (\mathcal{D}\{t_1\}, \mathcal{D}\{t_2\})$&
   $\mathcal{D}\{\pi_i~t\}$&$\coloneqq \pi_i~\mathcal{D}\{t\}$ \\
   $\mathcal{D}\{b\}~(b \in \{\mathbf{T},\mathbf{F}\})$ &$\coloneqq b$ &
   $\mathcal{D}\{\mathbf{if}~t~\mathbf{then}~t_1~\mathbf{else}~t_2\}$&$\coloneqq \mathbf{if}~\mathcal{D}\{t\}~\mathbf{then}~\mathcal{D}\{t_1\}~\mathbf{else}~\mathcal{D}\{t_2\}$ \\
   $\mathcal{D}\{\{t_1 \mapsto t_2\}\}$ &$\coloneqq \{\mathcal{D}\{t_1\} \mapsto \mathcal{D}\{t_2\}\}$ &
  $\mathcal{D}\{t_1 \mdoubleplus t_2\}$ &$\coloneqq \mathcal{D}\{t_1\} \mdoubleplus \mathcal{D}\{t_2\}$ \\
   $\mathcal{D}\{t_1[t_2]\}$ &$\coloneqq \mathcal{D}\{t_1\}[\mathcal{D}\{t_2\}]$ &
   $\mathcal{D}\{\sample~t\}$&$\coloneqq \mathcal{D}\{t\}$ \\
   $\mathcal{D}\{r\}$ &$\coloneqq (r, 0)$ &
   $\mathcal{D}\{\score~t\}$ &$\coloneqq \lambda \kappa. \haskdo \{y \gets \kappa(()); \return (\mathcal{D}\{t\} \times_\mathcal{D} y)\}$ \\
   $\mathcal{D}\{\return~t\}$&$\coloneqq \lambda \kappa. \kappa(\mathcal{D}\{t\})$ &
   $\mathcal{D}\{\haskdo~\{x \gets t; m\}\}$&$\coloneqq \lambda\kappa.\mathcal{D}\{t\}(\lambda x. \mathcal{D}\{\haskdo\{m\}\}(\kappa))$\\
   $\mathcal{D}\{\mathbf{normal}_{\text{REPARAM}}\}$&\begin{tabular}[t]{@{}l}$\coloneqq\lambda ((\mu,\mu'),(\sigma, \sigma')). \lambda \kappa. \haskdo \{$\\
   $\quad\quad \epsilon \gets \mathbf{normal}_{\text{REPARAM}}(0, 1);$\\
   $\quad\quad \kappa((\sigma\epsilon + \mu, \sigma'\epsilon + \mu'))$\\
   $\quad\}$
   \end{tabular} & 
   $\mathcal{D}\{\mathbf{normal}_{\text{REINFORCE}}\}$&\begin{tabular}[t]{@{}l}$\coloneqq\lambda ((\mu,\mu'), (\sigma, \sigma')). \lambda \kappa. \haskdo \{$\\
   $\quad\quad x \gets \mathbf{normal}_{\text{REINFORCE}}(\mu, \sigma);$\\
   $\quad\quad (y, y') \gets \kappa((x, 0));$\\
   $\quad\quad \llet~l' = \sigma'(\frac{1}{\sigma} + \frac{(y-\mu)^2}{\sigma^3}) + \mu' \frac{y-\mu}{\sigma^2};$\\
   $\quad\quad \return~(y, y'+yl')$\\
   $\quad\}$
   \end{tabular}\\
   $\mathcal{D}\{\mathbf{flip}_{\text{ENUM}}\}$&\begin{tabular}[t]{@{}l}$\coloneqq\lambda (p,p'). \lambda \kappa. \haskdo \{$\\
   $\quad\quad (y_T, y_T') \gets \kappa(\mathbf{T});$\\
   $\quad\quad (y_F, y_F') \gets \kappa(\mathbf{F});$\\
   $\quad\quad \llet~y=py_T + (1-p)y_F;$\\
   $\quad\quad \llet~y_1'=p'y_T + py_T';$\\
   $\quad\quad \llet~y_2'=(1-p)y_F' - p'y_F;$\\
   $\quad\quad \return~(y, y_1' + y_2')$\\
   %$\quad\quad x \gets \mathbf{flip}_{\text{ENUM}}(\mu, \sigma);$\\
   %$\quad\quad (y, dy) \gets \kappa((x, 0));$\\
   %$\quad\quad \llet~dl = d\sigma \times (\frac{1}{\sigma} + \frac{(y-\mu)^2}{\sigma^3}) + d\mu \times \frac{y-\mu}{\sigma^2};$\\
   %$\quad\quad \return~(y, dy+y\times dl)$\\
   $\quad\}$
   \end{tabular} & 
   $\mathcal{D}\{\mathbf{flip}_{\text{REINFORCE}}\}$&\begin{tabular}[t]{@{}l}$\coloneqq\lambda (p,p'). \lambda \kappa. \haskdo \{$\\
   $\quad\quad b \gets \mathbf{flip}_{\text{REINFORCE}}(p);$\\
   $\quad\quad (y, y') \gets \kappa(b);$\\
   $\quad\quad \llet~l'=\mathbf{if}~b~\mathbf{then}~\frac{p'}{p}~\mathbf{else}~\frac{p'}{p-1};$\\
   $\quad\quad \return (y, y' + yl')$\\
   $\quad\}$
   \end{tabular}
   \\
   % $\mathcal{D}\{\mathbf{normal}_{\text{REPARAM}}\}$&$\coloneqq \lambda(\mu, d\mu).\lambda(\sigma,d\sigma).\lambda\kappa.\haskdo \{\epsilon \gets \mathbf{normal}_{\text{REPARAM}}(0, 1); \kappa((\sigma \times \epsilon + \mu, d\sigma \times \epsilon + d\mu))\}$\\
   % $\mathcal{D}\{\mathbf{normal}_{\text{REINFORCE}}\}$&$\coloneqq \lambda(\mu, d\mu).\lambda(\sigma,d\sigma).\lambda\kappa.\haskdo \{x \gets \mathbf{normal}_{\text{REINFORCE}}(\mu, \sigma); (l, dl) \gets \kappa((x,0)); (p, dp) \gets \mathcal{D}\{\log\}; \return (l, dl + l \times dp)\}$\\
   \end{tabular}
\end{tabular}
}

    \caption{Monte Carlo gradient estimation as a program transformation from $\lambda_{\text{ADEV}}$ to $\lambda_{\text{ADEV}}$.}
    \label{fig:adev-transformation}
\end{figure}


==> fig/sec4-languages.tex <==
\begin{figure}
\begin{minipage}{0.45\textwidth}
{\footnotesize
\centering
    \textcolor{blue}{\textit{\textbf{Stochastic Probabilities}} ($\lambda_{\text{GenSP}}$)}
    \begin{align*}
    \text{Types }\type \, ::= \,&
        \text{Alg} \\
    \text{Terms }\ter \, ::= \,&
        \mathbf{importance} \mid \mathbf{marginal} \mid \mathbf{normalize} \\ %\mid
    \end{align*}

    \begin{mdframed}
        \centering
        \begin{tabular}{c}
           $ $ 
           \\\hline
           $\mathbf{importance} : G~\tau \to \NN \to \text{Alg}$
        \end{tabular}
        \quad
        \begin{tabular}{c}
           $ $ 
           \\\hline
           $\mathbf{marginal} : G~(D~\tau) \to (\tau \to \text{Alg}) \to D~\tau$
        \end{tabular}
        \quad
        \begin{tabular}{c}
           $ $ 
           \\\hline
           $\mathbf{normalize} : G~\tau \to \text{Alg} \to G~\tau$
        \end{tabular}
    \end{mdframed}

    \vspace{2mm}

    {\scriptsize{
    \centering
    $\sem{\text{Alg}} \coloneqq (\mathbb{T} \Rightarrow \text{Prob}~\RR) \Rightarrow \text{Prob}~\mathbb{T}$
    \quad
    $\sem{\mathbf{importance}} \coloneqq \lambda q. \lambda n. \lambda \rho. \lambda U. \int_{\mathbb{T}}q(du_1)\rho(dw_1) \cdots\int_{\mathbb{T}}q(du_n) \sum_{i=1}^n \delta_{u_i}(U)$
    $\sem{\mathbf{normal}_{\text{REPARAM}}} = \sem{\normal_{\text{REINFORCE}}} = \lambda (\mu, \sigma). \mathcal{N}(\mu, \sigma)$
    }}
    }
\end{minipage}\hfill%
\begin{minipage}{0.45\textwidth}
A thing
\end{minipage}
    \vspace{2mm}

    \caption{New types, typing rules, and denotations for our extension to $\lambda_{\text{Gen}}$.}
    \label{fig:syntax}
\end{figure}


==> fig/sec4-transform.tex <==
\begin{figure}
\scriptsize{
\begin{tabular}{ll}
    % Overall spec
   {Spec}  & \framebox{\textcolor{blue}{\textbf{\textit{Syntax}}}\;\;$\vdash_{\text{GenSP}} t : G~\tau \implies \vdash_{\text{ADEV}} \mathbf{density}\{t\} : \trace \to P~\RR$ \quad\quad\textcolor{blue}{\textbf{\textit{Semantics}}}\;\;$\sem{\mathbf{density}\{t\}} = \frac{d\sem{t}_1}{d\mathcal{B}_\mathbb{T}}$\quad\quad\quad\quad\quad\quad\quad\quad\quad} \\
   % Wrapper implementation
   \rule{0pt}{4ex}{Wrapper}  & $\mathbf{density}\{t\} \coloneqq \lambda u. \llet~(x, w, u') = \xi\{t\}(u)~\lin~\mathbf{if}~\textit{isempty}(u')~\mathbf{then}~w~\mathbf{else}~0$\\
   % Spec for helper
   \rule{0pt}{6ex}{Helper} $\xi$ & \framebox{\textcolor{blue}{\textbf{\textit{Syntax}}}\;\;$\Gamma \vdash_{\text{GEN}} t : \tau \implies \xi\{\Gamma\} \vdash_{\text{ADEV}} \xi\{t\} : \xi\{\tau\}$\quad\quad\quad\quad\quad \textcolor{blue}{\textbf{\textit{Semantics}}}\;\;$\forall (\gamma, \gamma') \in R^\xi_{\Gamma}, (\sem{t}(\gamma), \sem{\xi\{t\}}(\gamma')) \in R^{\xi}_\tau$}\\
   % Implementation on types
    \rule{0pt}{4ex}\;\textit{on types} & \begin{tabular}[t]{@{}l@{}l|l@{}l}
        $\xi\{\sigma\}$ &$\coloneqq \sigma$ & $R^\xi_\sigma$ &$\coloneqq \{(x, x) \mid x \in \sem{\sigma}\}$ \\
        $\xi\{D~\sigma\}$&$\coloneqq \sigma \to \RR$ & $R^\xi_{D~\sigma}$ &$\coloneqq \{(\mu, \rho) \mid \rho = \frac{d\mu}{d\mathcal{B}_\sigma}\}$\\
        $\xi\{\tau_1 \times \tau_2\}$&$\coloneqq \xi\{\tau_1\} \times \xi\{\tau_2\}$ & $R^\xi_{\tau_1 \times \tau_2}$ &$\coloneqq \{((x,y), (x',y')) \mid (x,x') \in R^\xi_{\tau_1} \wedge (y,y') \in R^\xi_{\tau_2}\}$\\
        $\xi\{\tau_1 \to \tau_2\}$&$\coloneqq \xi\{\tau_1\} \to \xi\{\tau_2\}$ & $R^\xi_{\tau_1 \to \tau_2}$ &$\coloneqq \{(f,g) \mid \forall (x,y) \in R^\xi_{\tau_1}, (f(x),g(y)) \in R^\xi_{\tau_2}\}$\\
        $\xi\{G~\tau\}$&$\coloneqq \trace \to \xi\{\tau\} \times \RR \times \trace$ & $R^\xi_{G~\tau}$ &\begin{tabular}[t]{@{}l}
        $\coloneqq \{((\mu,f),g) \mid \exists h. \forall u \in \mathbb{T}. (f(u), h(u)) \in R^\xi_{\tau} \; \wedge$ \\ 
        $\quad\quad\quad\quad\quad\quad\quad\quad\quad g = \lambda u. \llet~(u_1, u_2) = \textit{split}_\mu(u)~\lin (h(u), \frac{d\mu}{dB_\mathbb{T}}(u_1), u_2)\}$
        \end{tabular}\\
        % & & \text{where} $\mathbb{T}_\mu$&$\coloneqq \{u \in \mathbb{T} \mid \exists u' \in \mathbb{T}. \frac{d\mu}{d\mathcal{B}_\mathbb{T}}(u\mdoubleplus u') > 0\}, \mathbb{T}_\mu^*\coloneqq \lambda u. \text{argmax}_{\{u' \in \mathbb{T}_\mu \mid u' \subseteq u\}} |u'|$\\ % \forall_{\mu \otimes \mu} (u_1, u_2), u_1 = u_2 \vee \exists s \in u_1. s \in u_2 \wedge u_1[s] \neq u_2[s]$\\
        %& & \text{and} $\mathbb{T}_\mu^*$& $\coloneqq \lambda u. \text{argmax}_{\{u' \in \mathbb{T}_\mu \mid u' \subseteq u\}} |u'|$\\
        % & & \text{and} $\text{eat}_\mu$ & $\coloneqq \lambda u. u \setminus \mathbb{T}_\mu^*(u)$
    \end{tabular} \\
   % \rule{0pt}{4ex}\quad\textit{on types} & $\xi\{\sigma\} \coloneqq \sigma \;\mid\; \xi\{D~\sigma\} \coloneqq \sigma \to \RR \;\mid\; \xi\{\tau_1 \to \tau_2\} \coloneqq \xi\{\tau_1\} \to \xi\{\tau_2\}$ \\
   % Implementation on terms
   \rule{0pt}{4ex}\;\textit{on terms} & \begin{tabular}[t]{@{}l@{}l@{}l@{}l}
        $\xi\{()\}$ &$\coloneqq ()$ &
        %$\xi\{c\}$ &$\coloneqq c_\xi$\\
        $\xi\{x\}$ &$\coloneqq x$ \\
        $\xi\{\lambda x. t\}$ &$\coloneqq \lambda x. \xi\{t\}$ &
        $\xi\{t_1~t_2\}$ &$\coloneqq \xi\{t_1\}~\xi\{t_2\}$\\
        $\xi\{(t_1, t_2)\}$ &$\coloneqq (\xi\{t_1\}, \xi\{t_2\})$ &
        $\xi\{\pi_i~t\}$ &$\coloneqq \pi_i~\xi\{t\}$\\
        $\xi\{b\} (b \in \{\mathbf{T}, \mathbf{F}\})$ &$\coloneqq b$ &
        $\xi\{\mathbf{if}~t~\mathbf{then}~t_1~\mathbf{else}~t_2\}$ &$\coloneqq \mathbf{if}~\xi\{t\}~\mathbf{then}~\xi\{t_1\}~\mathbf{else}~\xi\{t_2\}$\\
        $\xi\{\normal_{\text{REPARAM}}\}$ &$\coloneqq \lambda \mu. \lambda \sigma. \lambda x. \frac{1}{\sigma\sqrt{2\pi}}e^{-\frac{1}{2}\left(\frac{x-\mu}{\sigma}\right)^2}$ &
        $\xi\{\normal_{\text{REINFORCE}}\}$ 
        &$\coloneqq \lambda \mu. \lambda \sigma. \lambda x. \frac{1}{\sigma\sqrt{2\pi}}e^{-\frac{1}{2}\left(\frac{x-\mu}{\sigma}\right)^2}$\\
        $\xi\{\flip_{\text{ENUM}}\}$ &$\coloneqq \lambda p. \lambda b. \mathbf{if}~b~\mathbf{then}~p~\mathbf{else}~1-p$ &
        $\xi\{\flip_{\text{REINFORCE}}\}$ 
        &$\coloneqq \lambda p. \lambda b. \mathbf{if}~b~\mathbf{then}~p~\mathbf{else}~1-p$\\
        $\xi\{\return~t\}$ &$\coloneqq \lambda u. (\xi\{t\}, 1, u)$ &
        $\xi\{\observe~t_1~t_2\}$ &$\coloneqq \lambda u. ((), \xi\{t_1\}(\xi\{t_2\}), u)$ \\
        $\xi\{\sample~t_1~t_2\}$ &\begin{tabular}[t]{@{}l}
        $\coloneqq \lambda u. \llet~(v,w,u')=\textit{pop}~u~\xi\{t_2\}$\\
        $\quad\quad\;\;\,\lin~(v,w\cdot\xi\{t_1\}(v), u')$
        \end{tabular} &
        $\xi\{\haskdo~\{x \gets t; m\}\}$ &\begin{tabular}[t]{@{}l}
        $\coloneqq \lambda u. \llet~(x,w,u')=\xi\{t\}(u)~\lin$\\
        $\quad\quad\;\;\,\llet~(y,v,u'') = \xi\{\haskdo\{m\}\}(u')~\lin$\\
        $\quad\quad\;\;\,(y,w\cdot v, u'')$
        \end{tabular}
   \end{tabular}\\
\end{tabular}
\vspace{1mm}
\hrule
\vspace{2mm}
\begin{tabular}{ll}
    % Overall spec
   {Spec}  & \framebox{\textcolor{blue}{\textbf{\textit{Syntax}}}\;\;$\vdash_{\text{GEN}} t : G~\tau \implies \vdash_{\text{ADEV}} \mathbf{sim}\{t\} : P~(\trace \times \RR)$ \quad \textcolor{blue}{\textbf{\textit{Semantics}}}\;\;$\sem{\mathbf{sim}\{t\}}(U) = \int \sem{t}_1(du) 1_U\!\left(u, \frac{d\sem{t}_1}{d\mathcal{B}_\mathbb{T}}(u)\right)$} \\
   % Wrapper implementation
   \rule{0pt}{4ex}{Wrapper}  & $\mathbf{sim}\{t\} \coloneqq \haskdo \{ (x, w, u) \gets \chi\{t\}; \return~(u, w)\}$\\
   % Spec for helper
   \rule{0pt}{6ex}{Helper} $\chi$ & \framebox{\textcolor{blue}{\textbf{\textit{Syntax}}}\;\;$\Gamma \vdash_{\text{GEN}} t : \tau \implies \chi\{\Gamma\} \vdash_{\text{ADEV}} \chi\{t\} : \chi\{\tau\}$\quad\quad\quad\textcolor{blue}{\textbf{\textit{Semantics}}}\;\; $\forall (\gamma, \gamma') \in R^\chi_{\Gamma}, (\sem{t}(\gamma), \sem{\chi\{t\}}(\gamma')) \in R^{\chi}_\tau$}\\
   % Implementation on types
    \rule{0pt}{4ex}\;\textit{on types} & \begin{tabular}[t]{@{}ll|ll}
        $\chi\{\sigma\}$ &$\coloneqq \sigma$ & $R^\chi_\sigma$ &$\coloneqq \{(x, x) \mid x \in \sem{\sigma}\}$ \\
        $\chi\{D~\sigma\}$&$\coloneqq P~(\sigma \times \RR)$ & $R^\chi_{D~\sigma}$ &$\coloneqq \{(\mu, \nu) \mid \nu(U) = \int \mu(du) \delta_{\left(u,\frac{d\mu}{d\mathcal{B}_\sigma}(u)\right)}(U)\}$\\
        $\chi\{\tau_1 \times \tau_2\}$&$\coloneqq \chi\{\tau_1\} \times \chi\{\tau_2\}$ & $R^\chi_{\tau_1 \times \tau_2}$ &$\coloneqq \{((x,y), (x',y')) \mid (x,x') \in R^\chi_{\tau_1} \wedge (y,y') \in R^\chi_{\tau_2}\}$\\
        $\chi\{\tau_1 \to \tau_2\}$&$\coloneqq \chi\{\tau_1\} \to \chi\{\tau_2\}$ & $R^\chi_{\tau_1 \to \tau_2}$ &$\coloneqq \{(f,g) \mid \forall (x,y) \in R^\chi_{\tau_1}, (f(x),g(y)) \in R^\chi_{\tau_2}\}$\\
        $\chi\{G~\tau\}$&$\coloneqq P~(\sem{\tau} \times \RR \times \trace)$ & $R^\chi_{G~\tau}$ &$\coloneqq \{((\mu,f),\nu) \mid \mu(\mathbb{T}) < 1 \vee \nu=\lambda U.\int\mu(du) 1_U(f(u), \frac{d\mu}{d\mathcal{B}_\mathbb{T}}(u), u)\}$
    \end{tabular} \\
   % \rule{0pt}{4ex}\quad\textit{on types} & $\xi\{\sigma\} \coloneqq \sigma \;\mid\; \xi\{D~\sigma\} \coloneqq \sigma \to \RR \;\mid\; \xi\{\tau_1 \to \tau_2\} \coloneqq \xi\{\tau_1\} \to \xi\{\tau_2\}$ \\
   % Implementation on terms
   \rule{0pt}{4ex}\;\textit{on terms} & \begin{tabular}[t]{@{}l@{}l@{}l@{}l}
        $\chi\{()\}$ &$\coloneqq ()$ &
        %$\xi\{c\}$ &$\coloneqq c_\xi$\\
        $\chi\{x\}$ &$\coloneqq x$ \\
        $\chi\{\lambda x. t\}$ &$\coloneqq \lambda x. \chi\{t\}$ &
        $\chi\{t_1~t_2\}$ &$\coloneqq \chi\{t_1\}~\chi\{t_2\}$\\
        $\chi\{(t_1, t_2)\}$ &$\coloneqq (\chi\{t_1\}, \chi\{t_2\})$ &
        $\chi\{\pi_i~t\}$ &$\coloneqq \pi_i~\chi\{t\}$\\
        $\chi\{b\} (b \in \{\mathbf{T}, \mathbf{F}\})$ &$\coloneqq b$ &
        $\chi\{\mathbf{if}~t~\mathbf{then}~t_1~\mathbf{else}~t_2\}$ &$\coloneqq \mathbf{if}~\chi\{t\}~\mathbf{then}~\chi\{t_1\}~\mathbf{else}~\chi\{t_2\}$\\
        $\chi\{\normal_{\text{REPARAM}}\}$ &\begin{tabular}[t]{@{}l}
        $\coloneqq \lambda (\mu, \sigma). \haskdo \{$\\
        $\quad\quad x \gets \normal_{\text{REPARAM}}~(\mu, \sigma);$\\
        $\quad\quad \llet~\rho = \frac{1}{\sigma\sqrt{2\pi}}e^{-\frac{1}{2}\left(\frac{x-\mu}{\sigma}\right)^2};$\\
        $\quad\quad\return (x, \rho)$\\
        $\quad\}$
        \end{tabular}&
        $\chi\{\normal_{\text{REINFORCE}}\}$ 
        &\begin{tabular}[t]{@{}l}
        $\coloneqq \lambda (\mu, \sigma). \haskdo \{$\\
        $\quad\quad x \gets \normal_{\text{REINFORCE}}~(\mu, \sigma);$\\
        $\quad\quad \llet~\rho = \frac{1}{\sigma\sqrt{2\pi}}e^{-\frac{1}{2}\left(\frac{x-\mu}{\sigma}\right)^2};$\\
        $\quad\quad\return (x, \rho)$\\
        $\quad\}$
        \end{tabular}\\
        $\chi\{\flip_{\text{ENUM}}\}$ &\begin{tabular}[t]{@{}l}
        $\coloneqq \lambda p. \haskdo \{$\\
        $\quad\quad b \gets \flip_{\text{ENUM}}~p;$\\
        $\quad\quad \llet~\rho = \mathbf{if}~b~\mathbf{then}~p~\mathbf{else}~1-p;$\\
        $\quad\quad\return (b, \rho)$\\
        $\quad\}$
        \end{tabular} &
        $\chi\{\flip_{\text{REINFORCE}}\}$ 
        &\begin{tabular}[t]{@{}l}
        $\coloneqq \lambda p. \haskdo \{$\\
        $\quad\quad b \gets \flip_{\text{REINFORCE}}~p;$\\
        $\quad\quad \llet~\rho = \mathbf{if}~b~\mathbf{then}~p~\mathbf{else}~1-p;$\\
        $\quad\quad\return (b, \rho)$\\
        $\quad\}$
        \end{tabular}\\
        $\chi\{\return~t\}$ &$\coloneqq \return (\chi\{t\}, 1, \{\})$ &
        $\chi\{\observe~t_1~t_2\}$ &$\coloneqq \bot ~ (\textcolor{red}{\textbf{compile-time error}})$ \\
        $\chi\{\sample~t_1~t_2\}$ &\begin{tabular}[t]{@{}l}
        $\coloneqq \haskdo \{$\\ 
        $\quad\quad (x,w) \gets \chi\{t_1\};$\\
        $\quad\quad \return (x, w, \{\chi\{t_2\} \mapsto x\})$\\
        $\quad \}$
        \end{tabular} &
        $\chi\{\haskdo~\{x \gets t; m\}\}$ &\begin{tabular}[t]{@{}l}
        $\coloneqq \haskdo \{$\\
        $\quad\quad (x, w, u_1) \gets \chi\{t\};$\\
        $\quad\quad (y, v, u_2) \gets \chi\{\haskdo\{m\}\};$\\
        $\quad\quad \mathbf{if} \textit{disj}(u_1, u_2)~\mathbf{then}$\\
        $\quad\quad\quad \return~(y,wv,u_1\mdoubleplus u_2)$\\
        $\quad\quad \mathbf{else}~\return~(y,0,\{\}))$\\
        $\quad\}$
        \end{tabular}
   \end{tabular}\\
\end{tabular}
}
    \caption{Traced simulation and density evaluation as program transformations from $\lambda_{\text{Gen}}$ to $\lambda_{\text{ADEV}}$.}
    \label{fig:gen-transformations}
    %\vspace{-7mm}
\end{figure}


==> fig/sec6-survey-table.tex <==
\begin{figure}[htb!]
\centering
\captionof{table}{A survey of variational objectives and their implementation using stochastic probabilities.}
\small
\begin{tabular}{| c | c |}
    \hline
    Method & Implementation \\
    \hline
    IWELBO \cite{bornschein_reweighted_2015} & $\lambda(\theta, \phi).\mathbb{E}(\haskdo \{ \log\textbf{density}\{\textbf{marginal} ~P ~(\textbf{SIR} ~Q ~N)\} ~(\theta, \phi) ~x \})$ \\
    HVI \cite{agakov_auxiliary_2004} & $\lambda(\theta, \phi).\mathbb{E}(\haskdo \{ \log \textbf{density}\{\textbf{marginal} ~P ~(\textbf{SIR} (\textbf{marginal} ~Q ~(\textbf{SIR} ~1)) ~1)\} ~(\theta, \phi) ~x\})$ \\
    IWHVI \cite{sobolev_importance_2019} & $\lambda(\theta, \phi).\mathbb{E}(\haskdo \{ \log \textbf{density}\{\textbf{marginal} ~P ~(\textbf{SIR} ~(\textbf{marginal} ~Q ~(\textbf{SIR} ~1)) ~M)\} ~(\theta, \phi) ~x\})$ \\
    DIWHVI \cite{sobolev_importance_2019} & $\lambda(\theta, \phi).\mathbb{E}( \haskdo\{\log \textbf{density}\{\textbf{marginal} ~P ~(\textbf{SIR} ~(\textbf{marginal} ~Q ~(\textbf{SIR} ~N)) ~M)\} ~(\theta, \phi) ~x\})$ \\
    \hline
\end{tabular}
\label{fig:spvi-table}
\end{figure}

==> fig/vae_transcript.tex <==
\begin{figure}[htb!]
    \includegraphics[width=\textwidth,height=0.5\textheight,keepaspectratio]{fig/vae/vae_architecture.png}
    \caption{Training variational autoencoders for generative modelling on MNIST. (Left) Model and guide graphical models: the model denotes a distribution over \textbf{z} and \textbf{img}, and the guide denotes a distribution over \textbf{z}, with \textbf{img} as input. (Right) Training curves for ELBO vs. IWAE ELBO variants. IWAE ELBOs achieve tighter bounds, potentially improving decoder performance, at the cost of guide posterior accuracy.}
    \label{fig:vae_transcript}
\end{figure}
